Conditional Density Estimation with Neural Networks: Best Practices and Benchmarks

Given a set of empirical observations, conditional density estimation aims to capture the statistical relationship between a conditional variable $\mathbf{x}$ and a dependent variable $\mathbf{y}$ by modeling their conditional probability $p(\mathbf{y}|\mathbf{x})$. The paper develops best practices for conditional density estimation for finance applications with neural networks, grounded on mathematical insights and empirical evaluations. In particular, we introduce a noise regularization and data normalization scheme, alleviating problems with over-fitting, initialization and hyper-parameter sensitivity of such estimators. We compare our proposed methodology with popular semi- and non-parametric density estimators, underpin its effectiveness in various benchmarks on simulated and Euro Stoxx 50 data and show its superior performance. Our methodology allows to obtain high-quality estimators for statistical expectations of higher moments, quantiles and non-linear return transformations, with very little assumptions about the return dynamic.

==> content/concistency_proofs.tex <==
\section{Universal Approximation Theorem for Mixture Density Networks}

\begin{theorem}[Universal function approximation theorem] \label{theorem:universal_fun_approx}
Let $\phi^{(m)}_\eta: \mathbb{R}^l \rightarrow \mathbb{R}$ with
\begin{equation}
   \phi^{(m)}_\eta(x) = \sum_{j=1}^m v_j \tau(w_j^\top x + b_j) ~, \quad v_j, b_j \in \mathbb{R}, ~ w_j \in \mathbb{R}^l \label{eq:perceptron}
\end{equation}
be a feed-forward network with one hidden layer of $m$ neurons and a nonconstant, bounded and continuous activation function $\tau: \mathbb{R} \rightarrow \mathbb{R}$. In that, $\eta \in H^{(m)}$ denotes the parameters $\eta = (v_1, ..., v_m, b_1, ..., b_m, w_1, ..., w_m)$  of the neural network. For all compact subsets $\mathcal{X} \subset \mathbb{R}^l$, continuous functions $f \in \mathcal{C}(\mathcal{X})$ and any $\epsilon > 0$, there exists a $n \in \mathbb{N}$ and $\eta \in H^{(m)}$ such that 
$$
| \phi^{(m)}_\eta(\rx) - f(\rx)| < \epsilon
$$

Proof. See \cite{Hornik1991a}
\end{theorem}

In the following, we extend the universal function approximation theorem to multidimensional functions, i.e. neural networks with multiple output neurons. First, we rephrase the expression in \ref{eq:perceptron} as
\begin{equation}
   \phi^{(m)}_\eta(x) = \bar{V}\tau(\bar{W} x + \bar{b}) ~, \quad \bar{V} \in \mathbb{R}^{1 \times m}, \bar{W} \in \mathbb{R}^{m \times l} , \bar{b}  \in \mathbb{R}^{m} \label{eq:perceptron}
\end{equation}
wherein the activation function $\tau : \mathbb{R}^{m} \rightarrow \mathbb{R}^{m}$ now acts as element-wise function. This allows us to easily extend the notations to neural networks $\rho^{(n)}_\theta: \mathbb{R}^l \rightarrow \mathbb{R}^k$ with k-dimensional real-valued output:
\begin{equation}
   \rho^{(n)}_\theta = V \tau(W x + b) ~, \quad V \in \mathbb{R}^{k \times n}, W \in \mathbb{R}^{n \times l} , b  \in \mathbb{R}^{n} \label{eq:perceptron}
\end{equation}
In that, $\theta = (V, W, b) \in \Theta^{(n)}$ represents the weights and biases of the neural network with $n$ hidden neurons and the corresponding the parameter space $\Theta^{(n)}$.

Before extending the function approximation theorem, we state a lemma that helps us to prove the following theorem. In fact, we show that any collection of $k$ neural networks with one output neuron can be replaced with one neural network with $k$ output neurons.

\begin{lemma} \label{lemma:multidim_nn}
Let $\rho_i(x), i=1,...,k$ denote the i-th output element of a function $\rho: \mathbb{R}^l \rightarrow \mathbb{R}^k$. For any tuple $(\phi^{(m_1)}_{\eta_1}, ..., \phi^{(m_k)}_{\eta_k})$ of one-layer neural networks $\phi^{(m_i)}_{\eta_i}: \mathbb{R}^l \rightarrow \mathbb{R}$ with one-dimensional output, there exists a neural network $\rho^{(n)}_\theta:  \mathbb{R}^l \rightarrow \mathbb{R}^k$ with $n = \sum_{i=1}^k m_i$ and $\theta \in \Theta^{(n)}$ so that $\rho^{(n)}_{\theta, i}(x) = \phi^{(m_i)}_{\eta_i} ~ \forall x \in \mathbb{R}^l$ and $i = 1, ..., k$.

Proof. We can construct such a network $\rho^{(n)}_\theta$ simply by combining the parameters of the $k$ one-dimensional neural networks as follows. First, we stack the weight matrices $\bar{W}_i$ and bias vectors $\bar{b}_i$ along their first dimension, i.e. let $W = [\bar{W}_1^\top, ...,\bar{W}_k^\top]^\top$ and $b = [\bar{b}_1^\top, ...,\bar{b}_k^\top]^\top$. This can be understood as concatenating the hidden layers of all $k$ networks. Second, we connect the hidden layer neurons originating from the $i$-th network with the $i$-th output neuron according to $\bar{V}_i$ and set the remaining connections equals zero. Accordingly, the weight matrix $V$ follows as:
$$
V = 
\begin{bmatrix}
    \bar{V}_{1,1} & \dots & \bar{V}_{1,m_1} & 0 & \cdots & 0 & \cdots & 0 \\
   0 & \dots & 0 & \bar{V}_{2,1}  & \cdots & 0 & \cdots & 0 \\
   \vdots & \vdots & \vdots & \vdots  & \ddots & \vdots & \ddots & \vdots \\
    0       &\dots & 0 & 0 & \cdots &\bar{V}_{k,1}& \cdots & \bar{V}_{k,m_k} \\
\end{bmatrix}  \in \R^{k \times n }
$$
This ensures that $\rho^{(n)}_{\theta, i}(x) = \bar{V}\tau(\bar{W} x + \bar{b}) = \phi^{(m_i)}_{\eta_i},~ i = 1, ..., k$. \qed
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Universal function approximation theorem for multidimensional output]
\label{theorem:universal_fun_approx_multidim}
Let $\rho^{(n)}_\theta: \mathbb{R}^l \rightarrow \mathbb{R}^k$ be a feed-forward network with one hidden layer containing $n$ neurons and a nonconstant, bounded and continuous activation function. In that, $\theta \in \Theta^{(n)}$ denotes the parameters of the neural network. For all compact subsets $\mathcal{X} \subset \mathbb{R}^l$, continuous functions $f \in \mathcal{C}(\mathcal{X})$ and any $\epsilon > 0$, there exists a $n \in \mathbb{N}$ and $\theta \in \Theta^{(n)}$ such that 
$$
\sup_{x \in \mathcal{X}} || \rho^{(n)}_\theta(\rx) - f(\rx)||_\infty < \epsilon
$$
%
%
Proof. Let $\phi^{(m)}_\eta: \mathbb{R}^l \rightarrow \mathbb{R}$ be a one-layer feed forward network with $m$ hidden neurons and one-output neuron. Also let $f_i(x): \mathbb{R}^l \rightarrow \mathbb{R}$ be the i-th component of $f \in \mathcal{C}(\mathcal{X})$. As a consequence of theorem \ref{theorem:universal_fun_approx}, for any $f \in \mathcal{C}(\mathcal{X})$ and $\epsilon > 0$, there exists a $k$-tuple $(\phi^{(m_1)}_{\eta_1}, ..., \phi^{(m_k)}_{\eta_k})$ of neural networks so that $\sup_{x \in \mathcal{X}} | \phi^{(m_i)}_\eta(x) - f_i(x)| < \epsilon$ for $ i = 1, ..., k$. Following from Lemma \ref{lemma:multidim_nn} there exists a neural network $\rho^{(n)}_\theta$ that is element-wise equal to the tuple of one-dimensional neural network functions, i.e. $\rho^{(n)}_{\theta, i}(x) = \phi^{(m_i)}_{\eta_i} ~ \forall x \in \mathbb{R}^l$ and $i = 1, ..., k$. Hence, for any $f \in \mathcal{C}(\mathcal{X})$ and $\epsilon > 0$ there exists a $\rho^{(n)}_{\theta}$ such that 
$$
\sup_{i=1, ..., k} \sup_{x \in \mathcal{X}} | \rho^{(n)}_{\theta, i}(x) - f_i(x)| = \sup_{x \in \mathcal{X}} || \rho^{(n)}_{\theta}(x) - f(x)||_{\infty} < \epsilon 
$$
\qed
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary} \label{corrolary:}
For all compact subset $\mathcal{X} \subset \mathbb{R}^l$, continuous functions $f \in \mathcal{C}(\mathcal{X})$ and any $\epsilon > 0$, there exists a $n_0 \in \mathbb{N} ~ \forall n > n_0 ~ \exists \theta \in \Theta^{(n)}$ such that 
$$
\sup_{x \in \mathcal{X}} || \rho^{(n)}_\theta(\rx) - f(\rx)||_\infty < \epsilon
$$
In other words, the approximation error tends to zero as the hidden layer size $n \rightarrow \infty$:
$$
\min_{\theta \in \Theta^{(n)}} \sup_{x \in \mathcal{X}} || \rho^{(n)}_\theta(\rx) - f(\rx)||_\infty \rightarrow 0
$$

Proof. We show the corollary by induction. From theorem \ref{theorem:universal_fun_approx_multidim} we know that $\forall \epsilon>0 ~ \exists n_0 \in \mathbb{N} ~ \exists \theta \in \Theta^{(n)}$ so that $\sup_{x \in \mathcal{X}} || \rho^{(n)}_\theta(\rx) - f(\rx)||_\infty < \epsilon$. 
Given any $\epsilon > 0$, assume there exists a set of parameters $\theta^{(n)} \in \Theta^{(n)}$ so that $\sup_{x \in \mathcal{X}} || \rho^{(n)}_\theta(\rx) - f(\rx)||_\infty < \epsilon$. Using the parameters $\theta^{(n)} = (V^{(n)}, W^{(n)}, b^{(n)})$ we can now construct a neural network $\rho^{(n+1)}_{\theta^{(n+1)}}$ with $n+1$ hidden layers that is functionally equal to $\rho^{(n)}_{\theta^{(n)}}$. To do so, we choose $V^{(n+1)} = [V^{(n)}, \mathbf{0}_k]$, $W^{(n+1)} = [{W^{(n)}}^\top, \mathbf{0}_l^\top]^\top$ and $b^{(n+1)} = [{b^{(n)}}^\top, \mathbf{0}_1^\top]^\top$ where $\mathbf{0}_k \in \mathbb{R}^{k \times 1}$ is a $k$-dimensional column vector of zeros, i.e. set all added weighs and biases to zero. 
This assures that $\rho^{(n)}_{\theta^{(n)}}(x) = \rho^{(n+1)}_{\theta^{(n+1)}} ~ \forall x \in \mathbb{R}^l$ and thus implies that there is a exists a $\rho^{(n+1)}_{\theta^{(n+1)}}$ with $\theta^{(n+1)} \in \Theta^{(n+1)}$ such that $\sup_{x \in \mathcal{X}} || \rho^{(n+1)}_{\theta^{(n+1)}} - f(\rx)||_\infty < \epsilon$.
The corollary follows by induction. \qed
\end{corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Universal approximation theorem for finite mixtures] \label{lemma:approx_thrm_finit_mixture}
Let $p \in C(\mathbb{R}^m)$ be a continuous probability density function. If $g \in C(\mathbb{R}^m)$ is also a continuous density, then, for any compact set $\mathcal{Y} \subset \mathbb{R}^m$ and and $\epsilon > 0$ there exists a finite mixture of the form
\begin{equation} \label{eq:finite_mixture}
    \hat{p}^{(k)}(y) = \sum_{i=1}^k w_i \frac{1}{\sigma_i^m} g \left( \frac{y-\mu_i}{\sigma_i}\right), \quad w_i \geq 0, ~\sum_{i=1}^k w_i = 1, ~ \mu_i \in \mathbb{R}^m, \text{and} ~ \sigma_i > 0
\end{equation}
such that 
\begin{equation*}
  \sup_{y \in \mathcal{Y}} |p(y) - \hat{p}^{(k)}(y)| < \epsilon
\end{equation*}
Proof. See \citet{Cheney2009} and \citet{Nguyen2016}
\end{lemma}

In the following we denote the parameters of a $k$-component mixture as 
$$\xi^{(k)} = (w_1, ..., w_k, \mu_1, ..., \mu_k, \sigma_1, ..., \sigma_k) \in \Xi^{(k)} \subseteq \mathbb{R}_{\geq 0}^k \times \mathbb{R}^{k \times m} \times \mathbb{R}_{>0}^k$$
Further, we write $\hat{p}(y; \xi^{(k)})$ to indicate the the parametrization of the mixture distribution. Mixture density networks comprise a neural network $\rho_\theta^{(n)}(x): \mathbb{R}^l \rightarrow \Xi^{(k)}$ that regresses onto the parameter space of the mixture distribution, outputting the parameters of $\hat{p}$ as a function of the conditional variable $x \in \mathbb{R}^l$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary} \label{corollary:finite_mixture_approx_thrm}
For any continuous probability density functions $p, g \in C(\mathbb{R}^m)$, any compact set $\mathcal{Y} \subset \mathbb{R}^m$ and $\epsilon > 0$, there exists a sequence of finite mixtures parameters $(\xi^{(k)})_{k \in \mathbb{N}}$ such that $\exists k_0 \in \mathbb{N} ~ \forall k > k_0$ 
\begin{equation}
  \sup_{y \in \mathcal{Y}} |p(y) - \hat{p}^{(k)}(y, \xi^{(k)})| < \epsilon \label{eq: cond_mixture_approx_thr}
\end{equation} 
In other words, there exists a sequence of finite mixtures $(\hat{p}^{(k)})_{k \in \mathbb{N}}$ so that the approximation error vanishes:
\begin{equation*}
  \sup_{y \in \mathcal{Y}} |p(y) - \hat{p}^{(k)}(y)| \rightarrow 0, ~ \text{as} ~ k \rightarrow \infty
\end{equation*}
%
Proof. We prove the corollary by induction. Following from lemma \ref{lemma:approx_thrm_finit_mixture}, for any $p \in C(\mathbb{R}^m)$ and $\epsilon > 0 ~ \exists k_0 ~ \exists \xi^{(k_0)} \in \Xi^{(k_0)}$ such that $\sup_{y \in \mathcal{Y}} |p(y) - \hat{p}^{(k)}(y, \xi^{(k)})| < \epsilon$.
Assume we have a $\xi^{(k)}$ that fulfills condition (\ref{eq: cond_mixture_approx_thr}), then we can construct a $\xi^{(k+1)}$ by adding $w_{k+1}=0$ and arbitrary $\mu_{k+1} \in \mathbb{R}^m, \sigma_{k+1} \in \mathbb{R}_{>0}$ to the tuple of mixture parameters. This ensures that $\hat{p}(y; \xi^{(k+1)}) = \hat{p}(y; \xi^{(k)}) ~ \forall y $ and implies that if there is a $\xi^{(k)}$ that fulfills (\ref{eq: cond_mixture_approx_thr}) there must be a $\xi^{(k+1)}$ so that the same condition holds. \qed
\end{corollary}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[MDNs are universal approximators of conditional densities]
Given the dimensionaliy of $x$ and $y$, i.e. $l = dim(\mathcal{X}) < \infty$ and $m = dim(\mathcal{Y}) < \infty$, by 
\begin{equation} \label{eq:cond_kn_MDN}
    \hat{\mathcal{P}}_{MDN} = \left\{\hat{p}_{\theta}^{(k, n)}: \hat{p}_{\theta}^{(k, n)}(y|x) = \hat{p}^{(k)}(y; \rho_\theta^{(n)}(x)) \quad k \in \mathbb{N}, n \in \mathbb{N}, \theta \in \Theta^{(n)} \right\}
\end{equation}
we denote the class of finite MDNs that resemble conditional probability densities: $\hat{p}_{\theta}: \mathbb{R}^l \times \mathbb{R}^m \rightarrow \mathbb{R}_+$.
Let $p \in \mathcal{C}(\mathbb{R}^l \times \mathbb{R}^m)$ be any continuous probability density. For any compact subset $\mathcal{Z} \subset \mathbb{R}^l \times \mathbb{R}^m$, and any $\epsilon > 0$ $\exists k_0 ~ \forall k > k_0 ~\exists n_0 ~ \forall n > n_0 ~ \exists \theta \in \Theta^{(n)}$ so that   
\begin{equation}
    \sup_{(x,y) \in \mathcal{Z}} | p(y|x) - \hat{p}^{(k,n)}_\theta(y|x)| < \epsilon
\end{equation}
%
In other, words there exists a nested series of $\hat{p}^{(k,n)}_\theta(y|x) \in \hat{\mathcal{P}}_{MDN}$ such that 
\begin{equation}
    \lim_{k \rightarrow \infty}  \lim_{n\rightarrow \infty} \sup_{(x,y) \in \mathcal{Z}} | p(y|x) - \hat{p}^{(k,n)}_\theta(y|x)| = 0
\end{equation}
Proof. The proof is structured as follows. First, we show that for any $\epsilon > 0$ there exists a sequence of mixture parameters $(\xi^{(k)})_{k \in \mathbb{N}}$ that yield a good approximation of $p$. Second, we then show that these mixture parameters can be approximated arbitrary well through a neural network. Finally, we show that the composition of the neural network map and the finite mixture in turn yields a good approximation of the conditional density $p$.

From corollary \ref{corollary:finite_mixture_approx_thrm} we know that for any $\epsilon > 0$ there exists a series of finite mixture parameters $(\xi^{(k)})_{k \in \mathbb{N}}$ such that $\exists k_0 ~ \forall k > k_0$ it holds that 
$$
\sup_{y \in \mathcal{Y}} |p(y) - \hat{p}^{(k)}(y, \xi^{(k)})| < \frac{\epsilon}{2} 
$$
Next, usining theorem

\end{theorem}

